A First Look at Fairness of Machine Learning Based Code Reviewer Recommendation

The fairness of machine learning (ML) approaches is critical to the reliability of modern artificial intelligence systems. Despite extensive study on this topic, the fairness of ML models in the software engineering (SE) domain has not been well explored yet. As a result, many ML-powered software systems, particularly those utilized in the software engineering community, continue to be prone to fairness issues. Taking one of the typical SE tasks, i.e., code reviewer recommendation, as a subject, this paper conducts the first study toward investigating the issue of fairness of ML applications in the SE domain. Our empirical study demonstrates that current state-of-the-art ML-based code reviewer recommendation techniques exhibit unfairness and discriminating behaviors. Specifically, male reviewers get on average 7.25% more recommendations than female code reviewers compared to their distribution in the reviewer set. This paper also discusses the reasons why the studied ML-based code reviewer recommendation systems are unfair and provides solutions to mitigate the unfairness. Our study further indicates that the existing mitigation methods can enhance fairness by 100% in projects with a similar distribution of protected and privileged groups, but their effectiveness in improving fairness on imbalanced or skewed data is limited. Eventually, we suggest a solution to overcome the drawbacks of existing mitigation techniques and tackle bias in datasets that are imbalanced or skewed.

==> figure/RQ1/average-skewk.tex <==
\begin{figure*}[!h]
    \begin{subfigure}{\textwidth}
        \input{figure/RQ1/corms/avg-skewk-corms}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \input{figure/RQ1/revfinder/avg-skewk-revfinder}
    \end{subfigure}
\newline
\caption{The average skew@K for the top K results in each project under CORMS and RevFinder, where K has a value of 4, 6, and 10. If the value of this measure is negative, it indicates that the recommendation in that dataset is unfair.}
\label{fig:avg-skewk}
\end{figure*}

==> figure/RQ1/average-spdk.tex <==
\begin{figure*}[!h]
    \begin{subfigure}{\textwidth}
        \input{figure/RQ1/corms/avg-spdk-corms}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \input{figure/RQ1/revfinder/avg-spdk-revfinder}
    \end{subfigure}
\newline
\caption{The average SPD for the top K results in each project under CORMS and RevFinder, where K has a value of 4, 6, and 10. The red lines represents the desired SPD threshold. If a value exceeds that threshold, it indicates that the recommendation in that project is unfair. \song{please fix the issue}}\mamad{Professor, should I bring back this figure? Because yesterday we decided to remove it since it has duplicate values with the table. Although I need to update the values in the figure.}
\label{fig:avg-spdk}
\end{figure*}

==> figure/RQ1/avg-ndkl.tex <==
\begin{figure}[!h]
\begin{center}
\begin{tikzpicture}
\pgfkeys{
         /pgf/number format/precision=2, 
        /pgf/number format/fixed,
        /pgf/number format/fixed
    }
\begin{axis}[
    ybar=4pt,
    ymin=0,    
    ymax=0.2,
    width=9cm,
    enlarge x limits=0.5,
    nodes near coords,
    nodes near coords align={vertical},
    nodes near coords style={font=\tiny\bfseries\color{black}},
    legend style={
            at={(0.64, 1)},
            anchor=north,
            legend columns=2,
            legend cell align=left,
            /tikz/every even column/.append style={column sep=0.5cm}
    },
    ylabel={Average NDKL},
    symbolic x coords={CORMS,RevFinder},
    xtick=data,
    x tick label style={ align=center},
    ]
\addplot[fill=red,fill opacity=1] coordinates {(CORMS,0.05) (RevFinder,0.07)};
\addplot[fill=blue,fill opacity=1] coordinates {(CORMS,0.09) (RevFinder,0.1)};
\addplot[fill=pink,fill opacity=1] coordinates {(CORMS,0.17) (RevFinder,0.09)};
\addplot[fill=green,fill opacity=1] coordinates {(CORMS,0.09) (RevFinder,0.09)};
\addplot[fill=yellow,fill opacity=1] coordinates {(CORMS,0.09) (RevFinder,0.08)};
\addplot[fill=cyan,fill opacity=1] coordinates {(CORMS,0.07) (RevFinder,0.07)};
\legend{BSSW, FreeCodeCamp, Node.js, Shopify, GetSentry, NIXCommunity}
\end{axis}
\end{tikzpicture}
\end{center}
\caption{This chart displays the average normalized discounted KL divergence (NDKL) for the results in each dataset. If the value of this metric is positive, it means that the recommendation results suffer from unfairness.}
\label{fig:avg-ndkl}
\end{figure}

==> figure/RQ1/corms/avg-skewk-corms.tex <==
\begin{tikzpicture}
    \pgfkeys{
         /pgf/number format/precision=2, 
        /pgf/number format/fixed,
        /pgf/number format/fixed
    }
    \begin{axis}[
        ybar=2pt,
        bar width=6pt,    
        width=8cm,    
        height=5cm,    
        ylabel={Average Skew@K},    
        xlabel={},    
        xtick={1,2,3},
        nodes near coords,
        nodes near coords align={vertical},
        nodes near coords style={font=\tiny\bfseries\color{black}},
        xticklabels={Top-4, Top-6, Top-10},  
        ymin=-3,    
        ymax=1,
        xmin=0.5,
        xmax=3.5,
        legend style={
            at={(0.5,-0.15)},
            anchor=north,
            legend columns=2,
            legend cell align=left,
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        title={CORMS}
    ]

    
    \addplot[fill=red,fill opacity=1] coordinates {
        (1, -0.38)
        (2, -0.57)
        (3, -0.22)
    };
    \addlegendentry{BSSW}
    
    \addplot[fill=blue,fill opacity=1] coordinates {
        (1, 0.24)
        (2, 0.61)
        (3, 0.29)
    };
    \addlegendentry{FreeCodeCamp}
    
    \addplot[fill=pink,fill opacity=1] coordinates {
        (1, -2.7)
        (2, -2.7)
        (3, -2.7)
    };
    \addlegendentry{Node.js}
    
    \addplot[fill=green,fill opacity=1] coordinates {
        (1, -1.04)
        (2, -0.62)
        (3, -0.36)
    };
    \addlegendentry{Shopify}

    
    \addplot[fill=yellow,fill opacity=1] coordinates {
        (1, -0.91)
        (2, -0.75)
        (3, -0.33)
    };
    \addlegendentry{GetSentry}
    
    \addplot[fill=cyan,fill opacity=1] coordinates {
        (1, -2.12)
        (2, -0.66)
        (3, -0.57)
    };
    \addlegendentry{NIXCommunity}


    
   

    % \addplot[xcomb, dashed, red, line width=2pt] coordinates {(0,50) (8,50)};
    % % \addlegendimage{dashed, pink, line width=2pt}
    % \addlegendentry{SPD Threshold}
    
    % \legend{BSSW, FreeCodeCamp, Node.js, Shopify, GetSentry, NIXCommunity}
    
    \end{axis}
\end{tikzpicture}

==> figure/RQ1/corms/avg-spdk-corms.tex <==
\begin{tikzpicture}[scale=0.65]
    \pgfkeys{
         /pgf/number format/precision=2, 
        /pgf/number format/fixed,
        /pgf/number format/fixed
    }
    \begin{axis}[
        ybar=3pt,
        enlarge y limits={upper=0.1},
        bar width=14pt,
        width=14cm,
        height=8cm,
        ylabel={Average SPD@K},    
        xlabel={},    
        xtick={1,2,3,4},
        xticklabels={BSSW, Node.js, Shopify, GetSentry}, 
        ymin=0,    
        ymax=1,
        xmin=0.5,
        xmax=5.5,
        legend style={
            at={(0.5,-0.15)},
            anchor=north,
            legend columns=-1,
            legend cell align=left,
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        title={CORMS}
    ]

    % \addplot[fill=red,fill opacity=1] coordinates {
    %     (1, 0.33)
        


    % };
    % \addlegendentry{Top-3}
    
    \addplot[fill=blue,fill opacity=1, nodes near coords,
        nodes near coords align={vertical},
        nodes near coords style={font=\tiny\bfseries\color{black}},] coordinates {
        (1, 0.01)
        (2, 1)
        (3, 0.92)
        (4, 0.74)
    };
    \addlegendentry{Top-4}
    
    % \addplot[fill=pink,fill opacity=1] coordinates {
    %     (1, 0.51)
    

    % };
    % \addlegendentry{Top-5}
    
    \addplot[fill=green,fill opacity=1, nodes near coords,
        nodes near coords align={vertical},
        nodes near coords style={font=\tiny\bfseries\color{black}},] coordinates {
        (1, 0.22)
        (2, 1)
        (3, 0.92)
        (4, 0.81)
    };
    \addlegendentry{Top-6}

    
    % \addplot[fill=yellow,fill opacity=1] coordinates {
    %     (1, 0.49)

    % };
    % \addlegendentry{Top-8}
    
    \addplot[fill=cyan,fill opacity=1, nodes near coords,
        nodes near coords align={vertical},
        nodes near coords style={font=\tiny\bfseries\color{black}},] coordinates {
        (1, 0.2)
        (2, 1)
        (3, 0.85)
        (4, 0.80)
    };
    \addlegendentry{Top-10}

    % \addplot[fill=cyan,fill opacity=1] coordinates {
    %     (1, 0.33)
    % };
    % \addlegendentry{Top-12}
    
    % spd thr BSSW
    \addplot[const plot, dashed, red, line width=1pt] coordinates {(0,0.11) (1.5,0.11)};

    % % spd thr FreeCodeCamp
    % \addplot[const plot, dashed, red, line width=1pt] coordinates {(1.5,0.82) (2.4,0.82)};

    % % spd thr Node.js
     \addplot[const plot, dashed, red, line width=1pt] coordinates {(2.5,0.69) (3.5,0.69)};

     % spd thr Shopify
     \addplot[const plot, dashed, red, line width=1pt] coordinates {(3.5,0.78) (4.5,0.78)};

     % spd thr GetSentry
     \addplot[const plot, dashed, red, line width=1pt] coordinates {(4.5,0.74) (5.5,0.74)};

    % % spd thr NIXCommunity
    % \addplot[const plot, dashed, red, line width=1pt] coordinates {(5.5,0.83) (6.5,0.83)};

    
    % \addlegendimage{dashed, pink, line width=2pt}
    % \addlegendentry{SPD Threshold}
    
    % \legend{BSSW, FreeCodeCamp, Node.js, Shopify, GetSentry, NIXCommunity}
    
    \end{axis}
\end{tikzpicture}

==> figure/RQ1/revfinder/avg-skewk-revfinder.tex <==
\begin{tikzpicture}
    \pgfkeys{
         /pgf/number format/precision=2, 
        /pgf/number format/fixed,
        /pgf/number format/fixed
    }
    \begin{axis}[
        ybar=2pt,
        bar width=6pt,    
        width=8cm,    
        height=5cm,    
        ylabel={Average Skew@K},    
        xlabel={},    
        xtick={1,2,3},
        nodes near coords,
        nodes near coords align={vertical},
        nodes near coords style={font=\tiny\bfseries\color{black}},
        xticklabels={Top-4, Top-6, Top-10},  
        ymin=-2.3,    
        ymax=1,
        xmin=0.5,
        xmax=3.5,
        legend style={
            at={(0.5,-0.15)},
            anchor=north,
            legend columns=2,
            legend cell align=left,
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        title={RevFinder}
    ]

    
    \addplot[fill=red,fill opacity=1] coordinates {
        (1, -0.36)
        (2, -0.21)
        (3, -0.19)
    };
    \addlegendentry{BSSW}
    
    \addplot[fill=blue,fill opacity=1] coordinates {
        (1, 0.79)
        (2, 0.47)
        (3, 0.0)
    };
    \addlegendentry{FreeCodeCamp}
    
    \addplot[fill=pink,fill opacity=1] coordinates {
        (1, -1.67)
        (2, -1.15)
        (3, -0.66)
    };
    \addlegendentry{Node.js}
    
    \addplot[fill=green,fill opacity=1] coordinates {
        (1, -1.34)
        (2, -0.86)
        (3, -0.45)
    };
    \addlegendentry{Shopify}

    
    \addplot[fill=yellow,fill opacity=1] coordinates {
        ((1, -0.93)
        (2, -0.32)
        (3, -0.07)
    };
    \addlegendentry{GetSentry}
    
    \addplot[fill=cyan,fill opacity=1] coordinates {
        (1, -2.05)
        (2, -1.44)
        (3, -0.17)
    };
    \addlegendentry{NIXCommunity}


    
   

    % \addplot[xcomb, dashed, red, line width=2pt] coordinates {(0,50) (8,50)};
    % % \addlegendimage{dashed, pink, line width=2pt}
    % \addlegendentry{SPD Threshold}
    
    % \legend{BSSW, FreeCodeCamp, Node.js, Shopify, GetSentry, NIXCommunity}
    
    \end{axis}
\end{tikzpicture}

==> figure/RQ1/revfinder/avg-spdk-revfinder.tex <==
\begin{tikzpicture}[scale=0.65]
    \pgfkeys{
         /pgf/number format/precision=2, 
        /pgf/number format/fixed,
        /pgf/number format/fixed
    }
    \begin{axis}[
        ybar=3pt,
        enlarge y limits={upper=0.1},
        bar width=14pt,
        width=14cm,
        height=8cm,
        ylabel={Average SPD@K},    
        xlabel={},    
        xtick={1,2,3,4,5,6},
        xticklabels={BSSW, FreeCodeCamp, Node.js, Shopify, GetSentry, NIXCommunity}, 
        ymin=0,    
        ymax=1,
        xmin=0.5,
        xmax=6.5,
        legend style={
            at={(0.5,-0.15)},
            anchor=north,
            legend columns=-1,
            legend cell align=left,
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        title={RevFinder}
    ]

    % \addplot[fill=red,fill opacity=1] coordinates {
    %     (1, 0.33)
        


    % };
    % \addlegendentry{Top-3}
    
    \addplot[fill=blue,fill opacity=1, nodes near coords,
        nodes near coords align={vertical},
        nodes near coords style={font=\tiny\bfseries\color{black}},] coordinates {
        (1, 0.40)
        (2, 0.75)
        (3, 0.86)
        (4, 0.84)
        (5, 0.77)
        (6, 0.98)
    };
    \addlegendentry{Top-4}
    
    % \addplot[fill=pink,fill opacity=1] coordinates {
    %     (1, 0.51)
    

    % };
    % \addlegendentry{Top-5}
    
    \addplot[fill=green,fill opacity=1, nodes near coords,
        nodes near coords align={vertical},
        nodes near coords style={font=\tiny\bfseries\color{black}},] coordinates {
        (1, 0.42)
        (2, 0.77)
        (3, 0.84)
        (4, 0.81)
        (5, 0.75)
        (6, 0.91)
    };
    \addlegendentry{Top-6}

    
    % \addplot[fill=yellow,fill opacity=1] coordinates {
    %     (1, 0.49)

    % };
    % \addlegendentry{Top-8}
    
    \addplot[fill=cyan,fill opacity=1, nodes near coords,
        nodes near coords align={vertical},
        nodes near coords style={font=\tiny\bfseries\color{black}},] coordinates {
        (1, 0.42)
        (2, 0.79)
        (3, 0.82)
        (4, 0.81)
        (5, 0.77)
        (6, 0.82)
    };
    \addlegendentry{Top-10}

    % \addplot[fill=cyan,fill opacity=1] coordinates {
    %     (1, 0.33)
    % };
    % \addlegendentry{Top-12}
    
    % spd thr BSSW
    \addplot[const plot, dashed, red, line width=1pt] coordinates {(0,0.22) (1.5,0.22)};

    % spd thr FreeCodeCamp
    \addplot[const plot, dashed, red, line width=1pt] coordinates {(1.5,0.82) (2.4,0.82)};

    % spd thr Node.js
    \addplot[const plot, dashed, red, line width=1pt] coordinates {(2.5,0.69) (3.5,0.69)};

    % spd thr Shopify
    \addplot[const plot, dashed, red, line width=1pt] coordinates {(3.5,0.78) (4.5,0.78)};

    % spd thr GetSentry
    \addplot[const plot, dashed, red, line width=1pt] coordinates {(4.5,0.74) (5.5,0.74)};

    % spd thr NIXCommunity
    \addplot[const plot, dashed, red, line width=1pt] coordinates {(5.5,0.83) (6.5,0.83)};

    
    % \addlegendimage{dashed, pink, line width=2pt}
    % \addlegendentry{SPD Threshold}
    
    % \legend{BSSW, FreeCodeCamp, Node.js, Shopify, GetSentry, NIXCommunity}
    
    \end{axis}
\end{tikzpicture}

==> sec/Patterntable.tex <==
% \begin{table*}[t!]
% \caption{Patterns for mining API constraints.\song{Nima: please correct the format of rules, and also add a column to show the id}}
% 	\label{tab:patterns}
% 	\setlength{\tabcolsep}{3pt} 
% 	\scalebox{0.9}{
% \begin{tabular}{ll}
% \toprule
% Rules & Example Sentences \\ \midrule
% \textless{}D\_type\small default=\textless{}value\small{} & int default=0 \\
% \textless{}D\_type\small or \textless{}D\_type\small{} & int or float \\
% \textless{}Structure\small of shape \textless{}(shape)\small{}, default=\textless{}value\small{} & array-like of shape (n\_samples,n\_features), default=None \\
% \textless{}Structure\_Enum\small of shape \textless{}(shape)\small{}, default=\textless{}value\small{} & \{array-like, sparse matrix\} of shape (n\_samples, n\_features), default=None \\
% \textless{}Structure\small of shape \textless{}(shape)\small or \textless{}(shape)\small{} & array-like of shape (n\_samples,n\_features) or (n\_samples,) \\
% \textless{}D\_type\small{}/\textless{}structure\small{} & params: dict \\
% \{Structure\_Enum\} & \{list, tuple, set\} \\
% \{Values\_Enum\} default=\textless{}value\small{} & \{‘text’, ‘diagram’\}, default=None \\
% \{Values\_Enum\} & \{‘text’, ‘diagram’\} \\
% \textless{}Size\small length of \{Structure\_Enum\} & 2-length sequence (tuple, list, …) \\
% \textless{}Dimension\small d \textless{}structure\small{} & 2d Array \\
% \textless{}value\small (def), \textless{}value\small{},.... or \textless{}value\small{} & ‘backward’ (default), ‘forward’, or ‘nearest’ \\
% \textless{}Structure\small of  \textless{}D\_type\small{} & tuple of ints \\
% \textless{}value\small or \textless{}value\small{} & \cellcolor[HTML]{FFFFFF}None or "sequence" \\
% \textless{}D\_type\small{},optional & (int,optional) \\
% \textless{}Structure\small{},optional & (array-like,optional) \\
% \textless{}D\_type\small or \textless{}value\small{} & int or “all” \\
% \cellcolor[HTML]{FFFFFF}\textless{}D\_type\small or \textless{}value\small default=\textless{}value\small{} & int or “all”, default=10 \\ \bottomrule
% \end{tabular}
% }
% \end{table*}


\begin{table*}[t!]
\caption{Rules for mining constraints from parametric pages of APIs.\song{add a new column between "No" and "Rules", group them into different types, i.e., structure, shape, data type, default value, and optionality}}
\label{tab:ruless}%\arun{Unlike that related paper , our designed rule can get all the constraints in a parametric sentence using one rule alone, so we cant group them based on each constraint.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
\toprule
No & Rules & Examples                   \\
\midrule
1 &  & \textless{}D\_type\textgreater \, default=\textless{}value\textgreater{} & int default=0                       \\
2  & \textless{}D\_type\textgreater \, or \textless{}D\_type\textgreater{}    & int or float                        \\
3 &
  \textless{}Structure\textgreater \, of shape \textless{}(shape)\textgreater{}, default=\textless{}value\textgreater{} &
  array-like of shape (n\_samples,n\_features), default=None \\
4 &
  \textless{}Structure\_Enum\textgreater \, of shape \textless{}(shape)\textgreater{}, default=\textless{}value\textgreater{} &
  \{array-like, sparse matrix\} \, of shape (n\_samples, n\_features), default=None \\
5 &
  \textless{}Structure\textgreater \, of shape \textless{}(shape)\textgreater \, or \textless{}(shape)\textgreater{} &
  array-like of shape (n\_samples,n\_features) \, or (n\_samples,) \\
6  & \textless{}D\_type\textgreater{}/\textless{}structure\textgreater{}   & params: dict                        \\
7  & \{Structure\_Enum\}                                                   & \{list, tuple, set\}                \\
8  & \{Values\_Enum\} default=\textless{}value\textgreater{}               & \{`text', `diagram'\}, default=None \\
9  & \{Values\_Enum\}                                                      & \{`text', `diagram'\}               \\
10 & \textless{}Size\textgreater length of \{Structure\_Enum\}             & 2-length sequence (tuple, list, …)  \\
11 & \textless{}Dimension\textgreater \, d \textless{}structure\textgreater{} & 2d Array                            \\
12 &
  \textless{}value\textgreater (def), \textless{}value\textgreater{}, .... or \textless{}value\textgreater{} &
  `backward' (default), `forward', or `nearest' \\
13 & \textless{}Structure\textgreater \, of \textless{}D\_type\textgreater{}  & tuple of ints                       \\
14 & \textless{}value\textgreater \, or \textless{}value\textgreater{}        & None or ``sequence''                  \\
15 & \textless{}D\_type\textgreater{}, optional                             & (int,optional)                      \\
16 & \textless{}Structure\textgreater{}, optional                           & (array-like,optional)               \\
17 & \textless{}D\_type\textgreater \, or \textless{}value\textgreater{}      & int or ``all''                        \\
18 &
  \textless{}D\_type\textgreater \, or \textless{}value\textgreater default=\textless{}value\textgreater{} & 
  int or ``all'', default=10 \\
  \bottomrule
\end{tabular}}
\end{table*}





==> sec/related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Code Reviewer Recommendation Systems}
Other than CORMS and RevFinder, there are many different studies and approaches for code reviewer recommendation \cite{correct-crr, hybrid-colab, reviewbot, WhoReview, chrev}. Rahman et al. proposed CORRECT, a code reviewer recommendation technique that considers a developer's relevant cross-project work history and experience in specialized technologies related to a pull request to establish their eligibility as a code reviewer. They have evaluated their approach on 10 commercial and six open-source projects. Compared to the previous state-of-the-art technique, CORRECT was superior. \cite{correct-crr}. Xia et al. offered a recommendation algorithm that measures implicit relations using a hybrid approach that combines a matrix factorization-based model with a neighborhood-based strategy. \cite{hybrid-colab}. Balachandran presented ReviewBot, a tool that automates code review with static analysis. They stated that static analysis tools help improve code reviews, according to a user research. Review Bot generates reviewer suggestions based on source code line change history, which was more accurate than a comparable system based on file change history \cite{reviewbot}. Chouchen et al. proposed WhoReview, a multi-objective search-based approach for identifying the desirable set of peer reviewers for code changes. They employ the Indicator-Based Evolutionary Algorithm (IBEA) to select reviewers who are familiar with the code change given their current workload. They have evaluated their approach on four open-source software projects, and their approach outperformed all the previous state-of-the-art approaches.\cite{WhoReview}. Bahrami Zanjani et al. presented cHRev, a method for automatically recommending code reviewers based on their prior contributions in previous code reviews. By using specific information from prior reviews, the approach outperforms existing approaches on three open-source systems and a commercial codebase at Microsoft. The approach included quantification of review comments and their recency, which improves performance over general review information or source code repository data \cite{chrev}.

\subsection{Fairness in Software Engineering}
There are some studies that address the problem of fairness in software engineering \cite{software-fairness-fse18, fairsquare, fairness-mcr}, but this problem has not been fully studied in software engineering research, especially in the topic of fairness, leaving the software systems vulnerable to fairness issues and discrimination \cite{software-fairness-fse18, software-fairness-survey}.
Albarghouthi et al. Brun and Meliou \cite{software-fairness-fse18} outlined a vision for how software engineering research may address fairness flaws and calls on the software engineering research community to act.  They argued that software fairness is identical with software quality and that different software engineering difficulties, such as requirements, specification, design, testing, and verification, must be addressed in order to tackle this problem. used program verification to validate decision-making program fairness. They simplified the problem to a series of weighted volume computation problems and solved them using an SMT solver. They employed these ideas in a tool called FairSquare, which is used to validate the fairness qualities of decision-making programs derived from real-world datasets. According to the results of the evaluation, the technique outperformed state-of-the-art probabilistic program analyses \cite{fairsquare}. 

As previously stated, there is no other study that addresses the fairness issue in code reviewer recommendation. There are, however, some research works \cite{fairness-mcr,crr-labeling-bias} on the issue of bias in code reviewer suggestion and fairness in the process of modern code review. For example, German et al. investigated whether modern code reviews are conducted fairly, using fairness theory to develop a framework for understanding how fairness affects code reviews. They proposed a framework for controlling social behavior in current code reviews, presents evidence of fairness problems in the code review processes, and provided guidance on dealing with unfairness in code reviews \cite{fairness-mcr}. As we can see, this study focuses on analyzing fairness in modern code review, not code reviewer recommendation systems. Moreover, in another study \cite{crr-labeling-bias}, Tecimer et al. concentrated on the issue of choosing appropriate code reviewers for effective code reviews. The issue was that the datasets used to train these systems could contain systematic labeling bias, making ground truth inaccurate. As a result, they proposed A new strategy for detecting and eliminating bias in code reviewer recommendation systems that enhanced the MRR of five examined approaches in two open-source project datasets. In this example, Although the focus of this study is code reviewer recommendation systems, the goal of this study is to fix bias caused by labeling errors in order to improve performance, not fairness. Our work is the first to look at how code reviewer recommendation algorithms systematically discriminate against particular protected groups and analyze fairness based on human-related qualities.


==> sec/setup.tex <==
\section{Experiment Setup}
\label{sec:experiment}

\subsection{Research Questions}
\label{sec:rq}

{We answer the following research questions to evaluate the performance of our proposed approaches.}

\noindent \textbf{RQ1: Is there any unfairness issues in recent state-of-the-art modern code reviewer recommendation systems?}
\vspace{4pt}


\noindent \textbf{RQ2: What type of bias do the code reviewer recommendation system have, and how does it impact the results leading to unfair recommendations?}
\vspace{4pt}



\noindent \textbf{RQ3: How to mitigate the bias/unfairness in the code reviewer recommendation systems? Are the current approaches for bias/unfairness mitigation effective for the code reviewer recommendation systems?}
\vspace{4pt}


In RQ1, we set out to ...  
In RQ2, we ....
In RQ3, we explore....
In RQ4, we ....  


\subsection{Experiment Data}
\label{sec:dataset}

\song{ present your experiment projects}


\subsection{Evaluation Measure} 
\label{sec:metric}

\song{the metrics for evaluation}


==> table/candidate-datasets.tex <==
\begin{table}[]
\centering
\caption{List of candidate datasets. The joyent dataset has only one female reviewer, so we exclude this dataset from our analysis.}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{\#} & \textbf{Dataset}        & \textbf{Female Ratio} & \textbf{\# Female Reviewers} \\ \hline
1  & nodejs\_annotated       & 0.13                  & 5                                \\ \hline
2  & bssw\_annotated         & 0.42                  & 7                                \\ \hline
3           & joyent\_annotated       & 0.01                  & 1                                \\ \hline
4  & nixcommunity\_annotated & 0.01                  & 2                                \\ \hline
5  & getsentry\_annotated    & 0.10                  & 8                                \\ \hline
6  & shopify\_annotated      & 0.09                  & 18                               \\ \hline
7  & freeCodeCamp\_annotated & 0.12                  & 2                                \\ \hline
\end{tabular}
\label{table:candidate-datasets}
\end{table}
